Probabilistic Self-supervised Learning via Scoring Rules Minimization

In this paper, we propose a novel probabilistic self-supervised learning via Scoring Rule Minimization (ProSMIN), which leverages the power of probabilistic models to enhance representation quality and mitigate collapsing representations. Our proposed approach involves two neural networks; the online network and the target network, which collaborate and learn the diverse distribution of representations from each other through knowledge distillation. By presenting the input samples in two augmented formats, the online network is trained to predict the target network representation of the same sample under a different augmented view. The two networks are trained via our new loss function based on proper scoring rules. We provide a theoretical justification for ProSMIN's convergence, demonstrating the strict propriety of its modified scoring rule. This insight validates the method's optimization process and contributes to its robustness and effectiveness in improving representation quality. We evaluate our probabilistic model on various downstream tasks, such as in-distribution generalization, out-of-distribution detection, dataset corruption, low-shot learning, and transfer learning. Our method achieves superior accuracy and calibration, surpassing the self-supervised baseline in a wide range of experiments on large-scale datasets like ImageNet-O and ImageNet-C, ProSMIN demonstrates its scalability and real-world applicability.

==> chapters/overview_method.tex <==



\subsection{Notation}

Let $N \in \mathbb{N}$ be the number of observations and let $D \in \mathbb{N}$ be the number of features.
Let $\boldsymbol{X} \triangleq\left[\boldsymbol{x}_1, \ldots, \boldsymbol{x}_N\right]^T \in \mathbb{R}^{N \times D}$ be the matrix of the observation vectors. 
\newline

Let $\boldsymbol{G} \in\left(\mathbb{R}^{+}\right)^{N \times N}$ be a matrix which describes the known pairwise positive relation between samples. 
$\boldsymbol{G}$ will always be symmetric, the diagonal will contain zeros and  $(\boldsymbol{G})_{i, j}>0$ will be equivalent to $x_i, x_j$ being semantically related.
\newline

The input for each model will be described as $G_j(\boldsymbol{X})$, meaning that a transformation via $\boldsymbol{G}$ will add noise and rotation to the original data set before being fed into a specific model.
This transformation will be randomly and the different transformations will be described by indices $1,..., t$.
There will be $s$ different transformations $G_1,...,G_s$ for the student and $t-s-1$ transformations $G_{s+1},...,G_t$ for the teacher model.
\newline

Let $\boldsymbol{Z} \in  \mathbb{R}^{N \times K}$ be a matrix of feature maps $f_\theta: \mathbb{R}^D \mapsto \mathbb{R}^K$ obtained from a model (e.g. deep neural network), meaning that $\boldsymbol{Z} = (f_\theta(\boldsymbol{x_1}),..., f_\theta(\boldsymbol{x_N}))^T$. 
\newline

Let  $\xi$ be the parameters for the teacher and let $\theta$ be the parameters for the student model.

%still the old draft
\subsection{Algorithm Overview}

Our approach involves training the student model to learn both a mean ($\mu$) and a variance ($\sigma^2$) using a strictly proper scoring rule. 
This assumes that the predictions of the student model follow an underlying normal distribution.

In the first step of our algorithm, we provide multiple augmented views of the data to both the student model (using $m$ views) and the teacher model (using $n-(m+1)$ views). 
We then apply a softmax activation to the student network and add a prediction head consisting of a mean and variance layer. 
Random noise $\epsilon \sim \mathcal{N}(0,1)$ is sampled, and the predictions $z_j = \mu + \epsilon \sqrt{\sigma^2}$ are generated, which are then used as samples in the scoring rule. 
This introduces stochastic behavior in the student model while enabling backpropagation with respect to the student.

For the teacher network, we apply centering in the batch and a softmax layer before passing the outputs into our scoring rule. 
The teacher is updated using exponential moving average and does not use backpropagation to reduce computation time.

By utilizing a strictly proper scoring rule and retaining the ability to calculate gradients as usual (as proven in \ref{bem_exchange}), we can infer that our algorithm will converge towards the desired minimum.

The complete algorithm is illustrated in Figure \ref{fig:algorithm}.


\begin{figure}[ht]
\centering
\includegraphics[width=8cm]{figures/reparameterised_appr_ssl.pdf}
\caption{Schematic depiction of the Algorithm.}
\label{fig:algorithm}
\end{figure}




%here starts the new draft

\subsection{Algorithm Overview}

We have developed a new algorithm, drawing inspiration from \citet{dino} and \citet{byol} in terms of the architectural design. Additionally, we have incorporated a loss function inspired by \citet{likelihood_free_inference}.

Let $N \in \mathbb{N}$ be the number of observations and let $D \in \mathbb{N}$ be the number of features.
Let $\boldsymbol{X} \triangleq\left[\boldsymbol{x}_1, \ldots, \boldsymbol{x}_N\right]^T \in \mathbb{R}^{N \times D}$ be the matrix of the observation vectors representing the data. 

Let $\boldsymbol{G} \in\left(\mathbb{R}^{+}\right)^{N \times N}$ be a matrix which describes the known pairwise positive relation between samples. 
$\boldsymbol{G}$ will always be symmetric, the diagonal will contain zeros and  $(\boldsymbol{G})_{i, j}>0$ will be equivalent to $x_i, x_j$ being semantically related.

The input for each model will be described as $G_j(\boldsymbol{X})$, meaning that a transformation via $\boldsymbol{G}$ will add noise and rotation to the original data set before being fed into a specific model.
This transformation will be randomly and the different transformations will be described by indices $1,..., t$.
There will be $s$ different transformations $G_1,...,G_s$ for the student and $t-s-1$ transformations $G_{s+1},...,G_t$ for the teacher model.

Let $\boldsymbol{Z}_{\theta} \in  \mathbb{R}^{N \times K}$ be a matrix of feature maps $f_\theta: \mathbb{R}^D \mapsto \mathbb{R}^K$ obtained from a model, meaning that $\boldsymbol{Z}_{\theta} = (f_\theta(\boldsymbol{x_1}),..., f_\theta(\boldsymbol{x_N}))^T$ for parameter $\theta$. 

Let  $\xi$ be the parameters for the teacher and let $\theta$ be the parameters for the student model.
Hence, we can describe the student model for a single input $G_{i}, i \in 1,...,s$ as $\boldsymbol{Z}_{\theta} \circ G_{i}(\boldsymbol{X})$.
Additionally we added a linear layer $h$ to the student network and created two prediction heads, one for the mean ($\mu$) and one for the variance ($\sigma^2$).

With the assumption that the predictions of the student model follow an underlying normal distribution, we used the reparametrization trick to generate samples from our student model.
We sampled random noise $\epsilon_{j} \sim N(0,1), $ and created a fixed number of predictions
\begin{align*}
    z_j = \mu \circ h \circ \boldsymbol{Z}_{\theta} \circ G_{i}(\boldsymbol{X}) + \epsilon_{j} \sqrt{\sigma^2 \circ h \circ \boldsymbol{Z}_{\theta} \circ G_{i}(\boldsymbol{X})}
\end{align*}
for each augmented view with $j \in 1,...,r$ and $r \in \mathbb{N}$.

We then fed the generated predictions as samples into a strictly proper Scoring Rule $S$, the Convex Adjusted Energy Score with $\beta = 1$, which can be found in Section \ref{adj_score}.
This introduces stochastic behavior in the student model while enabling backpropagation with respect to the student.
We updated student model via backpropagation minimizing the Scoring Rule.
This can be described as follows:
\begin{align*}
    \hat{\theta}:=\argmin_{\theta} J(\theta), \quad J(\theta) =\hat{S}(P_\theta, P_\xi)
\end{align*}
with the unbiased estimator of the Scoring Rule being the Convex Adjusted Energy Score: 
\begin{align*}
    \hat{S}(P_\theta, P_\xi) = 
    \dfrac{1}{N} \sum_{i=1}^{N} \!\left[ 
    \dfrac{2 \lambda}{r} \sum_{j=1}^{r} \Vert z_{j}^{i} - \phi_\xi^{i}\Vert^{\beta}_{2} -
    \frac{1- \lambda}{r(r-1)} \sum_{j,k = 1, j \neq k} \Vert z_{j}^{i} - z_{k}^{i} \Vert^{\beta}_{2} \!\right]
\end{align*}
where $\phi_\xi^{i}$ represents the teacher prediction for the $i$-th input.

As for the teacher model, we performed centering in each batch before passing the outputs into our scoring rule.
We updated the teacher using exponential moving average with the weights of the student and does not use backpropagation to reduce computation time.
The updates of the weights are performed as follows:
\begin{align*}
    \xi_0 &= \xi_0 \\
    \xi_t &= \alpha \theta_t + (1-\alpha)\xi_{t-1}, \quad t \in \mathbb{N}, \alpha \in [0,1]
\end{align*}



By utilizing a strictly proper scoring rule and retaining the ability to calculate gradients as usual (as proven in \ref{bem_exchange}), we can infer that our algorithm will converge towards the desired minimum.

The complete algorithm is illustrated in Figure \ref{fig:algorithm}.


\begin{figure}[ht]
\centering
\includegraphics[width=8cm]{figures/reparameterised_appr_ssl.pdf}
\caption{Schematic depiction of the Algorithm.}
\label{fig:algorithm}
\end{figure}



==> chapters/rebuttal.tex <==
\section{NeurIPS Rebuttal}

The theoretical justification appears to be straightforward. The theoretical result below Eq. (7) can be intuitively derived. However, the conclusion stated in Line 169 requires further discussion, as the arguments for converging to the minimum are not sufficiently substantiated.

Our used Scoring Rule is strictly proper, meaning that there exists a unique minimum (Appendix 9.2).
Additionally, we have shown that we can exchange gradients and expectations of our derivatives and hence can calculate them in a standard manner (Appendix 9.5.4).
Using Stochastic Gradient Descent, our algorithm will converge towards the minimum induced by the target networks' distribution.
This implies that our objective function operates in a way that effectively updates the weights in a favorable manner.




W1) The proposed probabilistic addition is rather simplistic (injecting non-learnable Gaussian noise).

A1) Simplicity is one of the strong points of this method.
The addition of a learnable mean and variance layer is easy to understand and implement.
This means that it can be easily applied in practice.
Although the injected Gaussian noise is not learned by any model parameters, it still proves to be stabilizing the algorithm and leading to better results.




W2) The proposed scoring rule seems to be unwieldy in practice (e.g., expensive to compute).

A2) Our proposed scoring rule is as expensive to compute as a regular energy score.
Compared to a regular loss function, without using samples and only updating the mean parameters, our loss function does take a lot of memory ($\mathcal{O}(r*N)$ instead of $\mathcal{O}(N)$, where $N$ is the number of data points and $r$ the number of samples).
This is the disadvantage for trying to learn a more meaningful representation including weights for the variance.
Without the additional computational effort it is not possible to learn the weights within the variance layer.
However, using our proposed scoring rule and choosing the number of samples carefully, leads to a relatively efficient calculation compared to other scoring rules (e.g., kernel score).





W3) The experiment did not illustrate sufficient delta over prior non-probabilistic methods in prediction or calibration.

A3) Although the margins over prior deterministic methods do not seem to be that large, it is still worth mentioning that our method also learns parameters not only for mean (prediction), but also for the variance.
Under the assumption of a Gaussian distribution one can easily provide confidence intervals and hence describe the uncertainty for the prediction.
This is a big advantage compared to earlier deterministic approaches and should be taken into account.


Complexity Analysis:



==> tables/ablation2.tex <==
%---------------------------------------------------
%     Table Transfer Learning
%---------------------------------------------------

\begin{table*}[!H]
\caption{\small \textbf{Important component for training}. We investigate the effect of each component on the Linear evaluation performance. The first line shows the best combination. PL. is the prediction layer. BN. is a Batch normalization layer.}
\label{table:transfer}
  \centering
  \scalebox{.7}{
  \begin{tabular}{l c c c c c }
   \toprule
    Energy (L1 loss) & Kernel score & Energy (L2-loss) & BN. & PL.  & Accuracy \\

    \midrule   
DINO~\cite{caron2021emerging}  & 99.0 & 90.5 & 72 & 98.5 \\     
i-BOT~\cite{zhou2021ibot}  & 99.1 & 90.7 & 73.7 & 98.6 \\   
\rowcolor{cyan!10}
ProSMin (ours)    &99.0&90.2  &72.5 &98.5  \\
    \bottomrule
  \end{tabular}
  }
\end{table*}

